Learning Networked Dynamical System Models with Weak Form and Graph Neural Networks

This paper presents a sequence of two approaches for the data-driven control-oriented modeling of networked systems, i.e., the systems that involve many interacting dynamical components. First, a novel deep learning approach named the weak Latent Dynamics Model (wLDM) is developed for learning generic nonlinear dynamics with control. Leveraging the weak form, the wLDM enables more numerically stable and computationally efficient training as well as more accurate prediction, when compared to conventional methods such as neural ordinary differential equations. Building upon the wLDM framework, we propose the weak Graph Koopman Bilinear Form (wGKBF) model, which integrates geometric deep learning and Koopman theory to learn latent space dynamics for networked systems, especially for the challenging cases having multiple timescales. The effectiveness of the wLDM framework and wGKBF model are demonstrated on three example systems of increasing complexity - a controlled double pendulum, the stiff Brusselator dynamics, and an electrified aircraft energy system. These numerical examples show that the wLDM and wGKBF achieve superior predictive accuracy and training efficiency as compared to baseline models. Parametric studies provide insights into the effects of hyperparameters in the weak form. The proposed framework shows the capability to efficiently capture control-dependent dynamics in these systems, including stiff dynamics and multi-physics interactions, offering a promising direction for learning control-oriented models of complex networked systems.

==> archive/intro.tex <==
% -----------------------------------------------
\section{Introduction}
% -----------------------------------------------
Powertrain electrification is a megatrend in vehicle design, leading to enhanced performance, new paradigms in safety and sustainability, and decreased lifetime costs \cite{Boglietti2009,Roberts2014b,Karimi2007,Gerstler2008,Park2021}. Electrified vehicle energy systems are characterized by complex nonlinear dynamics and are tightly coupled across multiple energy domains (e.g., electrical, thermal, mechanical). Modeling such complex systems stands as a formidable challenge in the field of system dynamics and control. The accuracy of these models not only influences the understanding and monitoring of system behaviors but also critically underpins the development of advanced control strategies.

% Data-driven modeling and control
Data-driven approaches have been successful in capturing unknown dynamics and patterns in complex systems \cite{schmid2010dynamic, berger2015estimation}, allowing for accurate dynamics prediction. However, these methods often produce nonlinear models requiring model-based control methods to be nonlinear as well, such as the iterative Linear Quadratic Regulator (iLQR) \cite{ma2022local} and Nonlinear Model Predictive Control (NMPC) \cite{gros2020linear}. These control methods can become increasingly computationally expensive as the number of system states increases, making them infeasible for real-time applications. Although some Reinforcement Learning (RL) approaches \cite{hu2022learning}, either model-based or model-free, can achieve good performance for nonlinear control, they often suffer from sampling inefficiency and lack of generalizability. Thus, there is a need for more efficient control methods that can be used with data-driven techniques to enable real-time control of nonlinear systems.

% Koopman
Control-oriented modeling approaches, particularly the Koopman Bilinear Form (KBF), offer significant advantages in capturing system dynamics while maintaining a structure amenable to control design \cite{Brunton2016, Mauroy2016, Surana2016, mauroy2020koopman, bevanda2021koopman, Goswami2022, Yu2023}. Koopman operator theory enables the embedding of nonlinear system dynamics in a lifted, higher-dimensional space where the dynamics are governed by a linear but possibly infinite-dimensional operator. This approach facilitates the application of linear or bilinear model-control techniques to the system, leveraging the expressive power and rigorous operator-theoretic guarantees of data-driven methods \cite{abraham2019active, Rosenfeld2021, schulze2022data}. Despite the success of data-driven methods for identifying Koopman operators, extending KBF to networked systems remains underexplored. Most existing approaches focus on Dynamic Mode Decomposition (DMD) and its variants, such as extended DMD with control (eDMDc) \cite{Proctor2016} and bilinear DMD (biDMD) \cite{Surana2016}. Mapping between physical and Koopman states and selecting the embedding representation pose significant challenges, particularly in maintaining predictive accuracy and generalizability. Recent approaches leverage deep neural networks to learn this mapping \cite{Li2017, Wang2021}, applying linear control methods \cite{Folkestad2022, shi2022deep}, showing improvements in model compactness and predictive accuracy. Despite these advances, the existing methods may not fully capture the complex interactions and dependencies among different components in a networked system. 
% Integrating KBF with geometric deep learning techniques remains an area ripe for exploration, as it has the potential to improve model performance and interpretability by encoding the relationships among different components of a complex system \cite{Battaglia2018, Zhou2020}. 

In many real-world applications, networked systems are often sparsely connected, so that each component only interacts with a small subset of other components. Conventional methods that consider full interactions among all components can be computationally inefficient and may not accurately represent the system's true dynamics. Moreover, these systems often exhibit heterogeneous connectivity, with uneven inputs and varying degrees of influence among components. Traditional machine learning algorithms, such as convolutional neural networks (CNNs), struggle with data defined on graphs due to their structured grid requirement, while graphs reside in non-Euclidean space and contain unordered nodes without fixed spatial locality. Integrating KBF with geometric deep learning (GDL) techniques has the potential to address these challenges by encoding the relationships and dependencies among different components of a complex system while efficiently handling sparse and heterogeneous connectivity \cite{Battaglia2018, Zhou2020}.

% Integrate graph into KBF
Graph-based representations naturally encode relationships and dependencies among different components of complex systems. Incorporating domain knowledge and system properties into graph structures can improve the capture of underlying dynamics and interactions, leading to more accurate and efficient models \cite{Yu2024c}. 
% Traditional machine learning algorithms, such as convolutional neural networks (CNNs), struggle with data defined on graphs due to their structured grid requirement, while graphs reside in non-Euclidean space and contain unordered nodes without fixed spatial locality. 
Graph Neural Networks (GNNs) \cite{Gori2005,Scarselli2009} have emerged as a powerful tool for modeling data defined on graphs, learning from both node-level and edge-level features to capture local and global patterns. They handle irregular and non-Euclidean data common in real-world applications, incorporating prior knowledge and complex data structures for better understanding and control of complex systems. GNN-based models have been successfully applied to complex physical simulations, such as in fluid dynamics \cite{Yu2022,Massegur2024}, weather systems \cite{Li2023,Yu2024b}, robotic control systems \cite{Sanchez2018, Li2019}, Hamiltonian mechanics \cite{Sanchez2019}, continuum dynamics \cite{Mrowca2018, Sanchez2020}, power system dynamics \cite{Karimi2021,Yu2024}, and traffic flow forecasting \cite{Guo2019,Bui2021}. While recent works incorporate graph-based representations into the  framework \cite{Fujii2019}, they do not explicitly consider the bilinear form of the Koopman operator or the effect of control inputs, which are essential for modeling and control of nonlinear systems \cite{Surana2016}.

% Learning dynamics from data
After selecting an appropriate model form, the next crucial step is to learn the system dynamics from available data. The learning process involves identifying the underlying relationships and dependencies among the system components and estimating the model parameters that best capture the observed behavior.
Several options exist for learning system dynamics from data, broadly categorized into discrete-time and continuous-time formulations. Discrete-time methods, such as autoregressive models \cite{Lutkepohl2005} and recurrent neural networks (RNNs) \cite{Hochreiter1997long}, map the system state from one time step to the next. These methods are generally computationally efficient and easy to implement, but the model cannot adapt to different time step sizes. This limitation poses significant challenges in various control scenarios, such as hierarchical Model Predictive Control (MPC), where the ability to handle multiple time step sizes is essential \cite{Yu2023}. In contrast, continuous-time methods learn the derivative of the system state with respect to time, offering a more natural and often more compact representation of underlying physical processes. 

Sparse Identification of Nonlinear Dynamics (SINDy) \cite{Brunton2016} is a continuous-time method that aims to identify the governing ordinary differential equations (ODEs) of a system from data. SINDy builds upon the idea of sparse regression, seeking to find a sparse set of nonlinear functions that best describe the system dynamics using a fixed library of candidate functions. One limitation of SINDy is the sensitivity to noise in the estimation of state derivatives. The numerical differentiation process used to approximate these derivatives can amplify noise in the input data, leading to inaccurate derivative estimates. This can result in the identification of incorrect or suboptimal governing equations, overfitting to noise, and reduced model interpretability. The weak SINDy method \cite{Messenger2021} \todo{full vs. partial} was proposed to address this issue, which formulates the problem in a weak form using test functions. The weak formulation has been shown to significant improve model performance in identifying system equations from data, by avoiding the amplification of errors resulting from numerical differentiation or noisy measurements \cite{Kaptanoglu2023}. Despite this improvement, the SINDy-based methods heavily rely on a fixed library of functions, which can limit their modeling capacity for complex, high-dimensional systems.

Deep learning-based models can automatically discover low-dimensional latent representations of high-dimensional systems, overcoming the limitations of fixed function libraries and enabling more efficient learning and prediction of complex, nonlinear behaviors \cite{Bengio2013}. Learning dynamics in a latent space offers several key advantages. First, it significantly reduces the dimensionality of the problem, leading to improved computational efficiency, particularly for systems with high-dimensional state spaces or intricate interactions. This reduction allows for faster training and inference, making real-time applications more feasible \cite{Hinton2006}. Second, for high-dimensional dynamical system, by projecting the system dynamics onto a lower-dimensional manifold, latent space representations can capture the essential features and underlying structure of the system, filtering out noise and irrelevant details \cite{Tenenbaum2000}. This focus on core dynamics can lead to models with improved generalizability and predictive accuracy.

Neural Ordinary Differential Equations (NODEs) \cite{Chen2018neural} and their graph-based variants \cite{Poli2019,Luo2023,Huang2023,Zang2020} are examples of deep learning models that learn continuous-time dynamics in a latent space. NODEs parameterize the derivative of the system state with respect to time using a neural network, allowing for the discovery of complex, nonlinear relationships between the state variables. Graph-based NODEs extend this idea by incorporating graph structures to capture the dependencies and interactions between different components of the system. While these models have shown impressive results in modeling complex systems, they also have limitations. NODEs can be computationally expensive, memory-intensive, and may introduce approximation errors and numerical instabilities during training \cite{Gholami2019anode, Zhuang2020adaptive}. This drawback is particularly prounced in the case of stiff systems, characterized by the presence of multiple timescales and fast-evolving dynamics, which can pose significant challenges to numerical integration and gradient computation in NODEs \cite{Wanner1996solving}.

% Contribution
% To address these limitations, we propose a novel deep learning approach that combines geometric deep learning and Koopman theory, trained using a weak formulation. 

To address these limitations and bridge the gap in the literature, we propose a novel approach that combines geometric deep learning and Koopman theory to efficiently model complex, networked systems with sparse and heterogeneous connectivity. The proposed model leverages the expressiveness of deep learning while preserving system structure through graph-based representations, enabling accurate capture of the complex dynamics and interactions among different components in a networked system. However, learning the model from data can be challenging due to the presence of noise and the potential for numerical instabilities, particularly in stiff systems. To address this issue, we propose a novel weak formulation for training the model, which improves performance, robustness, and efficiency in learning complex system dynamics. Our main contributions are as follows:
\begin{compactenum}
\item We introduce the Weak Form Latent Dynamics Model (wLDM), a general deep learning framework that leverages a weak formulation for training. The wLDM offers improved performance and robustness as compared to baseline methods, enabling faster and more stable training even for stiff systems.
% and noisy data.
\item Building upon the wLDM, we propose the Weak Form Graph Koopman Bilinear Form (wGKBF) model, which incorporates graph-based representations and KBF dynamics. The wGKBF model efficiently captures the complex dynamics of networked systems, such as a simulated electric aircraft energy system, by leveraging the expressiveness of deep learning while preserving system structure through graph-based representations.
\item We demonstrate the effectiveness of the proposed wLDM method, including its wGKBF variant, through three example systems of increasing complexity - a controlled double pendulum, the Brusselator chemical reaction, and an electric aircraft energy system. The results highlight the capability of the proposed frameworks to accurately model complex systems with improved efficiency and robustness as compared to existing approaches.
\end{compactenum}

% Data-driven methods for identifying the Koopman models have gained considerable attention due to the strong expressive power and the rigorous operator-theoretic guarantees \cite{abraham2019active,Rosenfeld2021, schulze2022data}. The learned linear system on the embedded space is readily amenable for linear or bilinear control techniques. 
% Conventionally, the possible representation of the embedding is given as a predefined dictionary \cite{Goldschmidt2021,Kaiser2021,Klus2022}.
% However, finding the mapping between the physical and Koopman states and selecting the embedding representation remains a challenging task, especially in terms of maintaining the predictive accuracy and generalizability.
 
% Recent approaches leverage deep neural networks to learn this mapping \cite{Li2017, Wang2021}, applying linear control methods \cite{Folkestad2022, shi2022deep}, showing improvements in model compactness and predictive accuracy.  Despite these advances, the existing methods may not fully capture the complex interactions and dependencies among different components in a networked system. Integrating KBF with geometric deep learning techniques remains an area ripe for exploration, as it has the potential to improve model performance and interpretability by encoding the relationships and dependencies among different components of a complex system \cite{Battaglia2018, Zhou2020}.

% % Paper org
% The rest of the paper is organized as follows. Section II presents the problem statement, the weak formulation training approach, and the wLDM framework. Section III describes the incorporation of KBF and GNN into wLDM, resulting in the wGKBF framework. Section IV presents numerical experiments, comparing our approach to existing methods and demonstrating its performance on three dynamical systems of increasing complexity. Finally, Section V concludes the paper and discusses potential future work.

%% Archive

% % Graph
% Graph-based representations have been shown to improve model performance and interpretability by encoding the relationships and dependencies among different components of a complex system \cite{Battaglia2018,Zhou2020}. Graphs provide a natural way to encode the relationships and dependencies among different components of a complex system. By incorporating domain knowledge and system properties into the graph structure, models can better capture the underlying dynamics and interactions. This leads to more accurate and efficient models, as the graph structure helps to constrain the search space and guide the learning process (\hl{cite Kuramoto paper}).

% % GNN
% The Graph Neural Network (GNN) \cite{Gori2005,Scarselli2009}, a recent variant of deep learning models, has emerged as a powerful tool for the modeling of data defined on graphs. These models can learn from both node-level and edge-level features, allowing for the capture of local and global patterns. Moreover, graph-based models can handle irregular and non-Euclidean data, which is common in many real-world applications. The ability to incorporate prior knowledge and handle complex data structures makes graph-based modeling a promising approach for understanding and controlling complex systems. The GNN-based models have been successfully applied to complex physical simulations, e.g. fluid dynamics \cite{Yu2022,Massegur2024}, robotic control systems \cite{Sanchez2018, Li2019}, Hamiltonian mechanics \cite{Sanchez2019}, continuum dynamics \cite{Mrowca2018, Sanchez2020}, power system dynamics \cite{Karimi2021,Yu2024}, and traffic flow forecasting \cite{Guo2019,Zhao2020,Bui2021}. While recent works incorporate graph-based representations into the DMD framework \cite{Fujii2019}, they do not explicitly consider the bilinear form of the Koopman operator or the effect of control inputs, which are essential for modeling and control of nonlinear systems \cite{Surana2016}.

% Sparse Identification of Nonlinear Dynamics (SINDy) \cite{Brunton2016} is ... SINDy has limited expressiveness due to its reliance on a fixed library of functions and can be sensitive to noise in the estimation of state derivatives. To address this issue, the weak SINDy method \cite{Messenger2021} has been proposed, which formulates the problem in a weak form using test functions. The weak formulation has been shown to significant improve model performance in identifying system equations from data, by avoiding the amplification of errors resulting from numerical differentiation or noisy measurements \cite{Kaptanoglu2023}. Nonetheless, wSINDy approach still relies on a fixed library of functions, limiting its modeling capacity. 

% Despite the success of data-driven methods for identifying Koopman operators, there is a lack of existing work on extending KBF to networked systems. Most approaches in the literature are based on Dynamic Mode Decomposition (DMD) and its variants, such as extended DMD with control (eDMDc) \cite{Proctor2016} and bilinear DMD (biDMD) \cite{Surana2016}. While recent works incorporate graph-based representations into the DMD framework \cite{Fujii2019}, they do not explicitly consider the bilinear form of the Koopman operator or the effect of control inputs, which are essential for modeling and control of nonlinear systems \cite{Surana2016}.

% Deep learning-based models \cite{Lusch2018,Greydanus2019,Regazzoni2024} have demonstrated superior expressivity in modeling high-dimensional, intricate, and nonlinear systems by automatically discovering low-dimensional latent dynamics. The motivation behind learning the dynamics in a latent space is to improve computational efficiency and capture the essential features of the system by reducing dimensionality \cite{Bengio2013}. This is particularly advantageous for systems with high-dimensional state spaces or complex, nonlinear behaviors. The choice of latent space dimensionality is a crucial hyperparameter that balances the trade-off between model complexity and information loss. A smaller latent dimension leads to a more compact representation but may result in a loss of information, while a larger latent dimension can capture more complex dynamics but may increase computational cost and the risk of overfitting. In practice, the optimal latent dimension can be determined through cross-validation or based on prior knowledge of the system's intrinsic dimensionality.

% existing approaches like Neural ODEs (NODEs) \cite{Chen2018neural} or its graph-based variations \cite{Poli2019,Luo2023,Huang2023,Zang2020}, and Sparse Identification of Nonlinear Dynamics (SINDy) \cite{Brunton2016} have limitations. NODEs can be computationally expensive, memory-intensive, and introduce approximation errors and numerical instabilities during training, especially  \cite{Gholami2019anode, Zhuang2020adaptive}.

% Powertrain electrification is a megatrend in vehicle design, offering enhanced performance, safety, sustainability, and decreased lifetime costs \cite{Boglietti2009,Roberts2014b,Karimi2007,Gerstler2008,Park2021}. However, electrified vehicle energy systems are characterized by complex nonlinear dynamics and tight coupling across multiple energy domains (e.g., electrical, thermal, mechanical), making modeling and control a formidable challenge. Data-driven approaches have been successful in capturing unknown dynamics and patterns in complex systems \cite{schmid2010dynamic, berger2015estimation}, but the resulting nonlinear models often require computationally expensive control methods, such as iterative Linear Quadratic Regulator (iLQR) \cite{li2004iterative} or Nonlinear Model Predictive Control (NMPC) \cite{gros2020linear}, which may be infeasible for real-time applications. While Reinforcement Learning (RL) approaches \cite{hu2022learning} can achieve good performance on nonlinear control, they often suffer from sampling inefficiency and lack of generalizability.

% % Continuous formulation
% In the realm of dynamic modeling, continuous models stand out for offering several advantages over discrete models. One key benefit is their adaptability to different time steps, which facilitates timescale analysis \cite{Chen2018neural}. This flexibility allows for the investigation of system behavior at various temporal resolutions, enabling a more comprehensive understanding of the underlying dynamics \cite{Garnier2003}. Moreover, continuous models can capture the smooth evolution of system states, providing a more natural and accurate representation of real-world processes \cite{Brunton2016b}.
% Continuous models also enable the use of powerful mathematical tools from calculus and differential equations, which can lead to more efficient and accurate numerical simulations \cite{Quarteroni2017}. Furthermore, the use of continuous models aligns well with the physical laws governing many complex systems, such as conservation principles and constitutive equations \cite{Willcox2021}. By leveraging the advantages of continuous models, we can develop more robust and informative representations of complex systems, ultimately leading to improved control and optimization strategies \cite{Proctor2016, Surana2016}.

% % NODE
% Neural Ordinary Differential Equations (Neural ODEs) are a continuous-time analog of deep neural networks that have gained attention for their ability to model complex dynamical systems \cite{Chen2018neural}. In a Neural ODE, the derivative of the hidden state is parameterized by a neural network, allowing the model to learn the dynamics of the system from data \cite{Dupont2019augmented}. However, training Neural ODEs with discrete data poses challenges. The standard approach involves using an ODE solver to compute the gradients of the loss function with respect to the model parameters, which requires the numerical integration of the ODE backwards in time (adjoint method) \cite{Pontryagin2018mathematical}. This process can be computationally expensive, memory-intensive, and can introduce approximation errors and numerical instabilities \cite{Gholami2019anode, Zhuang2020adaptive}.

% % SINDy, wSINDy
% Sparse Identification of Nonlinear Dynamics (SINDy) is a data-driven approach for identifying nonlinear dynamical systems from data \cite{Brunton2016}. It relies on a library of candidate functions, typically polynomials, to represent the system dynamics. The method then applies sparse regression techniques to select the most relevant terms from the library, resulting in a parsimonious model. However, SINDy has some limitations. First, its expressiveness is limited by the choice of the function library, which is often based on polynomials. This can lead to suboptimal performance when modeling complex, high-dimensional systems. Second, SINDy estimates the derivative of the state variables from potentially noisy data, which can introduce errors in the model identification process. To address this issue, the weak SINDy method \cite{Messenger2021} has been proposed, which formulates the problem in a weak form using test functions. While this approach improves robustness to noise, it still relies on a fixed library of functions, limiting its modeling capacity.

% % KBF with graph
% Despite the success of data-driven methods for identifying Koopman operators, there is a lack of existing work on combining Graph Koopman Bilinear Form (KBF) with deep learning. Most approaches in the literature are based on Dynamic Mode Decomposition (DMD) and its variants, such as extended DMD with control (eDMDc) \cite{Proctor2016} and bilinear DMD (biDMD) \cite{Surana2016}. These methods aim to identify the Koopman operator from data using a predefined set of observables, often based on polynomials or time-delay embeddings. However, they do not leverage the expressiveness and flexibility of deep learning models, which have shown great success in learning complex representations from data. Recently, there have been several works that incorporate graph-based representations into the DMD framework \cite{Fujii2019,} These approaches demonstrate the benefits of combining graph-based representations with DMD, capturing the intrinsic structure and interactions of the system. However, they do not explicitly consider the bilinear form of the Koopman operator or the effect of control inputs, which are essential for modeling and control of nonlinear systems \cite{Surana2016}.

--------------------






% Learning dynamics from data
After selecting an appropriate model form, the next step is to learn the system dynamics from available data. % The learning process involves identifying the underlying relationships and dependencies among the system components and estimating the model parameters that best capture the observed behavior.
The algorithms for learning dynamics are broadly categorized into discrete-time and continuous-time formulations. Discrete-time methods, such as autoregressive models \cite{Lutkepohl2005} and Recurrent Neural Networks \cite{Hochreiter1997long}, map the system state from one time step to the next. These methods are easy to implement, but may have highly nonlinear model forms, that are inconvenient for controller design.  Furthermore, it is either difficult or computationally inefficient to adapt the model to different time step sizes. This limitation poses significant challenges in various control scenarios, such as hierarchical MPC, where the ability to handle multiple time step sizes is essential \cite{Yu2023}. In contrast, continuous-time methods learn the time derivative of the states, offering a more natural and often more compact representation of underlying dynamical processes, especially when the underlying physics is governed by differential equations. 





A representative and widely used method in this category is the Sparse Identification of Nonlinear Dynamics (SINDy) \cite{Brunton2016}. The SINDy builds upon the idea of sparse regression, seeking to find a minimal set of nonlinear functions that best describe the system dynamics via an ordinary differential equation (ODE). The SINDy algorithm is relatively easy to implement as it only requires an iterative process of linear regressions. However, one limitation of SINDy is the sensitivity to the error of estimated state time derivatives, and inaccurate derivative estimates can result in the identification of incorrect or suboptimal governing equations. The weak SINDy (wSINDy) method \cite{Messenger2021} addresses this issue by re-formulating the linear regression problem using the so-called weak form.  The weak form uses a set of test functions to replace the time derivatives with numerical integrals, and thus bypassing the need for the derivative estimates that may be numerically unstable.
The wSINDy has been shown to significantly improve model performance in identifying system equations from data, by avoiding the amplification of errors resulting from numerical differentiation or noisy measurements \cite{Kaptanoglu2023}. Despite this improvement, the SINDy still heavily relies on a fixed library of functions, usually polynomials, that suffer from the curse of dimensionality; this characteristics fundamentally limits its modeling capacity for complex, high-dimensional systems, such as the networked systems.

Deep learning-based models can automatically discover low-dimensional latent representations of high-dimensional systems, overcoming the limitations of fixed function libraries and enabling more efficient learning and prediction of complex, nonlinear behaviors \cite{Bengio2013}. Learning dynamics in a latent space offers several key advantages. First, it significantly reduces the dimensionality of the problem, leading to improved computational efficiency, particularly for systems with high-dimensional state spaces or intricate interactions. This reduction allows for faster training and inference, making real-time applications more feasible \cite{Hinton2006}. Second, for high-dimensional dynamical system, by projecting the system dynamics onto a lower-dimensional manifold, latent space representations can capture the essential features and underlying structure of the system, filtering out noise and irrelevant details \cite{Tenenbaum2000}. This focus on core dynamics can lead to models with improved generalizability and predictive accuracy.
There is indeed an extension of wSINDy to a latent dynamics formulation using dimension reduction techniques, such as autoencoders \cite{Tran2024}.  However, in this approach, the dimension reduction and dynamics learning are performed in a sequential manner, and the dynamics still employ a fixed library of functions, which may suffer from lack of expressiveness. 
 Furthermore, the latent dynamics extension \cite{Tran2024} did not account for control inputs.





Hence, an alternative continuous-time formulation that is more promising for networked systems is the Neural Ordinary Differential Equations (NODEs) \cite{Chen2018neural} and their graph-based variants \cite{Poli2019,Zang2020,Luo2023,Huang2023}.  The NODEs are examples of deep learning models that learn continuous-time dynamics in a latent space. The NODEs parameterize the time derivative of states using a neural network, allowing for the discovery of complex, nonlinear relationships between the state variables. Graph-based NODEs extend this idea by incorporating graph structures to capture the interactions among the components of a networked system.
While these models have shown promising results in modeling complex systems, the main challenge is in the learning of such models.  Unlike SINDy, the NODEs rely on highly nonlinear and non-convex optimizations.  Furthermore, the gradient computation of NODEs, as needed in the learning process, can be numerically unstable and thus computationally expensive and memory-intensive \cite{Gholami2019anode, Zhuang2020adaptive}. This drawback is particularly pronounced in the case of stiff systems \cite{Kim2021stiff}, which may result in completely wrong models or even the failure of learning.  Hence the bottleneck of stiffness is highly undesirable for the learning of dynamics for networked systems, which are often stiff due to the multiple timescales.


==> archive/method.tex <==

% The direct approach solves for the parameters $\vtQ$ such that the discretized model fits the observed data points $\hvy_i$, and transform the continuous dynamical system into a discrete set of algebraic equations, thereby facilitating the use of established numerical optimization techniques which are typically robust and well-developed.

% Conversely, the indirect approach formulates the continuous-time adjoint equations and optimization problem first, and then discretizes the resulting optimality conditions \cite{Hinze2009}. The continuous-time adjoint equations are derived using the Hamiltonian function and the adjoint state, and the optimality conditions are obtained by setting the variations of the augmented objective functional to zero. These continuous-time optimality conditions are then discretized using appropriate numerical schemes. The indirect approach often results in numerical difficulties during optimization because it directly handles the continuous nature of the dynamics and adjoint equations, and the obtained gradients are typically more accurate. 

% One straightforward approach to solving the optimization problem Eq. \eqref{eqn:opt} is to use the continuous adjoint method, which introduces adjoint states (or "costates") governed by an adjoint ODE \cite{Bradley2019}. However, the adjoint ODE is often numerically stiff, making it challenging to solve in practice. Alternatively, discretization methods can be employed, categorized as "discretize-then-optimize" (direct) or "optimize-then-discretize" (indirect) approaches. In direct methods, we convert the ODE constraints \eqref{eqn:opt_ode} to algebraic constraints, and solve the resulting equality-constrained optimization using standard algorithms. 

% However, the continuous-time adjoint equations and optimality conditions can be much more complex to derive and implement compared to the direct approach.
% The NODEs have emerged as a promising indirect approach, leveraging neural networks to parameterize the dynamics and observation functions in a continuous-time setting. However, training NODEs can be computationally expensive and prone to numerical instabilities. To address these challenges, this paper focuses on the weak form,  a direct approach that reformulates the optimization problem using integral constraints and test functions, aiming to develop a more efficient and stable framework for inferring the parameters of nonlinear dynamical systems. In the following sections, we will discuss the general ideas behind NODEs and the weak form, then propose the Weak Form Latent Dynamics Model (wLDM), a general deep learning architecture that learns the dynamics of a system in a latent space, trained using the weak form.

% \subsection{Neural Ordinary Differential Equations}\label{sec:node}

% Neural Ordinary Differential Equations \cite{Chen2018neural} have emerged as a prominent indirect approach to learning the dynamics and observation functions of a system in a continuous-time setting. NODEs leverage the expressive power of neural networks to parameterize these functions, offering a flexible and data-driven approach to modeling complex, nonlinear systems.

% In the context of the problem statement in Eq.\eqref{eqn:system}, NODEs represent the dynamics function $\vf$ and the observation function $\vg$ as neural networks. The dynamics of the hidden state $\vh(t)$ in NODEs are described by the ordinary differential equation $\dot{\vh}=\vf(\vh, \vu;\vtQ)$. To obtain the hidden state at a future time $t_1$, the ODE is solved using a numerical integrator. The observation function $\vg$ maps the hidden state $\vh$ to the observed output $\vy$, i.e., $\vy = \vg(\vh,\vu;\vtQ)$. 
% % Training a NODE involves optimizing the parameters $\vtQ$ to minimize a loss function $\cL$, which measures the discrepancy between the predicted outputs and the true observations. The optimization problem can be formulated as:
% % \begin{subequations}\label{eqn:node}
% % \begin{align}
% % \min_\vtQ &\ J(\vtQ; \cD) = \int_{t_1}^{t_L} \norm{\vg(\vh,\vu;\vtQ) - \hvy^2} dt \\
% % \text{s.t.} &\ \dot{\vh}=\vf(\vh, \vu;\vtQ), \quad \vh(0) = \vh_0(\vtQ)
% % \end{align}
% % \end{subequations}
% The NODEs are trained by employing the adjoint method outlined in \ref{sec:indirect}, which efficiently computes the gradients of the loss function with respect to the parameters $\vtQ$.


% The observation function $\vg$ maps the hidden state $\vh$ to the observed output $\vy$, i.e., $\vy = \vg(\vh,\vu;\vtQ)$. Training a NODE involves optimizing the parameters $\vtQ$ to minimize a loss function $\cL$, which measures the discrepancy between the predicted outputs and the true observations. The optimization problem can be formulated as:
% \begin{subequations}\label{eqn:node}
% \begin{align}
% \min_\vtQ &\ \cL(\vtQ; \cD) = \int_{t_1}^{t_L} \norm{\vg(\vh,\vu;\vtQ) - \hvy^2} dt \\
% \text{s.t.} &\ \dot{\vh}=\vf(\vh, \vu;\vtQ), \quad \vh(0) = \vh_0(\vtQ)
% \end{align}
% \end{subequations}

% To train NODEs, the adjoint method \cite{Pontryagin2018mathematical} is employed to efficiently compute the gradients of the loss function with respect to the parameters $\vtQ$. The adjoint method introduces an adjoint state $\va(t) = \frac{\partial\cL}{\partial\vh}$, which is governed by another ODE that is solved backward in time:
% \begin{equation}
% \dot{\va} = -\va^T \frac{\partial \vf}{\partial \vh}(\vh, \vu, t)
% \end{equation}
% with the terminal condition $\va(t_L) = 0$.

==> archive/weak.tex <==
The weak formulation is a direct approach that reformulates the optimization problem by converting the ODE constraints into integral constraints using test functions. This approach can lead to a more efficient and stable training process compared to the continuous adjoint method. 

Following the approach in \cite{Messenger2021}, we introduce a set of test functions ${\phi_i(t)}_{i=1}^N$ defined on the time interval $[a,b]$, such that $\phi_i(t)=0$ for $t\notin[a,b]$ and $\phi_i$ satisfies the boundary conditions:
\begin{equation}\label{eqn_tst_bc}
\phi_i(a)=\phi_i(b)=0
\end{equation}

The ODE for dynamics can be converted to the weak form,
\begin{equation}\label{eqn_wf}
    - \int_a^b \dot{\phi}_i \vx dt = \int_a^b \phi_i \vf(\vx,\vu;\vtq) dt
\end{equation}
where the time derivative of $\vx$ is eliminated through integration-by-parts (resulting end values of $\vx$ are eliminated the boundary conditions of $\phi_i$).

The optimization problem \eqref{eqn_opt} is now
\begin{subequations}\label{eqn_opt_int}
\begin{align}\label{eqn_opt_obj}
    \min_\vtq &\ J(\vtq;\cD) \\\label{eqn_opt_ic}
    \text{s.t.} &\ - \int_a^b \dot{\phi}_i\vx dt = \int_a^b \phi_i\vf(\vx,\vu;\vtq) dt,\quad i=1,2,\cdots,N
\end{align}
\end{subequations}

Next we discretize the integrals in \eqref{eqn_opt_int} based on the data set $\cD$, and convert the optimization to a conventional equality-constrained problem.  Note that for any integrable functions, $g(t)$, given data pairs $\{(t_k,g(t_k))\}_{k=1}^K$, $a\leq t_1<t_2<\cdots<t_K\leq b$, one can perform numerical integration,
\begin{equation}
    \int_a^b g(t) dt \approx \sum_{i=1}^K v_kg(t_k) \equiv \vg^\mathbf{v}
\end{equation}
where $v_k$ are weights at time stations $t_k$, and
\begin{gather}
    \vg=[g(t_1),g(t_2),\cdots,g(t_K)]^T,\quad \mathbf{v}=[v_1,v_2,\cdots,v_K]^T
\end{gather}
The choice of $t_k$ will be discussed later.

Via numerical integration, the objective function is approximated as
\begin{align}\nonumber
    J(\vtq;\cD) &= \int_{t_1}^{t_L} \norm{\vh(\vx,\vu;\vtq)-\tvy}^2 dt \\\nonumber
    &\approx \sum_{k=1}^K v_k\norm{\vh_k-\tvy_k}^2 \\\label{eqn_wf_obj}
    &\equiv \tr((\vH-\tvY)\mathbf{v}(\vH-\tvY)^T)
\end{align}
where $\vh_k=\vh(\vx_k,\vu_k;\vtq)$, $\vH=[\vh_1,\vh_2,\cdots,\vh_K]$, and $\tvY=[\tvy_1,\tvy_2,\cdots,\tvy_K]$; $\mathbf{v}=\diag(\mathbf{v})$; $\tr()$ means matrix trace.

Similarly, for \eqref{eqn_opt_ic}, the left hand side of the $i$th constraint is,
\begin{equation}
    - \int_a^b \dot{\phi}_i\vx dt \approx -\sum_{k=1}^K v_k\dot{\phi}_i(t_k)\vx_k \equiv \vX\vd_i
\end{equation}
where $\vX=[\vx_1,\vx_2,\cdots,\vx_K]$ and
$
    \vd_i = [v_1\dot{\phi}_i(t_1),v_2\dot{\phi}_i(t_2),\cdots,v_K\dot{\phi}_i(t_K)]^T
$.

The right hand side is,
\begin{equation}
    \int_a^b \phi_i\vf(\vx,\vu;\vtq) dt \approx -\sum_{k=1}^K v_k\phi_i(t_k)\vf_k \equiv \vF\vc_i
\end{equation}
where $\vf_k=\vf(\vx_k,\vu_k;\vtq)$, $\vF=[\vf_1,\vf_2,\cdots,\vf_K]$ and
$
    \vc_i = [v_1{\phi}_i(t_1),v_2{\phi}_i(t_2),\cdots,v_K{\phi}_i(t_K)]^T
$.

The total of $N$ integral constraints can be written compactly as
\begin{equation}\label{eqn_wf_cons}
    \vX\vD = \vF(\vX,\vU;\vtq)\vC
\end{equation}
where $\vD=[\vd_1,\vd_2,\cdots,\vd_N]$ and $\vC=[\vc_1,\vc_2,\cdots,\vc_N]$, and we explicitly write the dependence of $\vF$ on states, inputs and parameters.

Up to this point, from \eqref{eqn_opt_obj} and \eqref{eqn_opt_wf}, we have obtained an optimization problem with algebraic equality constraints,
\begin{subequations}\label{eqn_opt_wf}
\begin{align}
    \min_\vtq &\ \tr((\vH-\tvY)\mathbf{v}(\vH-\tvY)^T) \\
    \text{s.t.} &\ \vX\vD = \vF(\vX,\vU;\vtq)\vC
\end{align}
\end{subequations}
To solve \eqref{eqn_opt_wf}, one can use standard algorithms such as interior point method and augmented Lagrangian method.  Yet, there are two potential challenges:
\begin{compactenum}

    \item High computational cost due to the large number of constraints; note that \eqref{eqn_opt_wf} is a matrix equation having ${n_x\times N}$ variables.
    \item Additional computational cost due to the high-dimensional intermediate variable $\vX\in\bR^{n_x\times K}$, since one needs to solve for $\vX$ to evaluate the objective $J$.
    \item Strong non-convexity caused by the nonlinearity in $\vf$, that may result in failure of convergence to $\vtq$ of the true system.
\end{compactenum}
We will attempt to address these challenges in the following sections.

\subsubsection{Choice of Test Functions}
The number of constraints $N$ depends on the choice of test functions ${\phi_i}$. One intuitive choice is:
\begin{equation}
\phi^I(t)=(t-a)^j(t-b)^k
\end{equation}
Another choice is based on the Jacobi polynomials, denoted $P_n^{(\alpha,\beta)}(\tau)$, $\tau\in[-1,1]$, that is orthogonal with respect to a weight function, $w^{(\alpha,\beta)}(\tau)=(1-\tau)^\alpha(1+\tau)^\beta$, and
\begin{equation}
    \int_{-1}^1 P_n^{(\alpha,\beta)}(\tau)P_m^{(\alpha,\beta)}(\tau)w^{(\alpha,\beta)}(\tau) d\tau = K_n^{(\alpha,\beta)} \delta_{nm}
\end{equation}
where $K_n^{(\alpha,\beta)}$ is a scaling factor and $\delta_{nm}$ the Dirac delta.  Using Jacobi polynomials, we choose the test functions to be
\begin{equation}
    \phi_i^J(t) = P_i^{(1,1)}(\tau) w^{(1,1)}(\tau)
\end{equation}
where $\tau = (t-(a+b)/2) / ((b-a)/2)$.  Note that $w^{(1,1)}(\tau)=(1-\tau^2)$ guarantees the satisfaction of the boundary conditions. Intuitively, Jacobi polynomials may achieve better convergence in representing the trajectory $\vx(t)$ when compared to the simplistic choice of $\phi_i^I$, which are not orthogonal.

\subsubsection{Choice of Numerical Integration Scheme}
The integration scheme determines the size of intermediate variables, especially $K$. One approach is to directly use time stations in the dataset $\cD$, which may lead to a large number of intermediate variables. An alternative is to approximate the true $\vx$ by a set of basis functions ${\psi_m}{m=1}^M$, $M\ll L$:
\begin{equation}\label{eqn_exp}
\vx(t) \approx \sum{m=1}^M \vs_m\psi_m(t) \equiv \vS\vty(t)
\end{equation}
where $\vs_m$ are coefficients of expansion, $\vS=[\vs_1,\vs_2,\cdots,\vs_M]$, and $\vty=[\psi_1,\psi_2,\cdots,\psi_M]^T$. This approach reduces the dimension of the intermediate variables. Using the expansion, the modified optimization formulation becomes:
\begin{subequations}\label{eqn_opt_exp}
\begin{align}
\min_{\vtq} &\ J(\vtq;\cD) \\
\text{s.t.} &\ \vS\hat{\vD} = \vF(\vS\vtY,\vU;\vtq)\vC
\end{align}
\end{subequations}
where $\hat{\vD}=[\hat{\vd}_1,\hat{\vd}_2,\cdots,\hat{\vd}_N]$ and $\vtY=[\vty(t_1),\vty(t_2),\cdots,\vty(t_K)]$.

This weak formulation approach addresses the challenges of high computational cost and strong non-convexity by reducing the number of constraints and intermediate variables, while maintaining the accuracy of the numerical integration.
